The DESI One-Percent Survey: Exploring the Halo Occupation Distribution of Luminous Red Galaxies and Quasi-Stellar Objects with AbacusSummit

We present the first comprehensive Halo Occupation Distribution (HOD) analysis of the DESI One-Percent survey Luminous Red Galaxy (LRG) and Quasi-Stellar Object (QSO) samples. We constrain the HOD of each sample and test possible HOD extensions by fitting the redshift-space galaxy 2-point correlation functions in 0.15 < r < 32 Mpc/h in a set of fiducial redshift bins. We use AbacusSummit cubic boxes at Planck 2018 cosmology as model templates and forward model galaxy clustering with the AbacusHOD package. We achieve good fits with a standard HOD model with velocity bias, and we find no evidence for galaxy assembly bias or satellite profile modulation at the current level of statistical uncertainty. For LRGs in 0.4 < z < 0.6, we infer a satellite fraction of fsat = 11+-1%, a mean halo mass of log10 Mh = 13.40+0.02-0.02, and a linear bias of blin = 1.93+0.06-0.04. For LRGs in 0.6 < z < 0.8, we find fsat = 14+-1%, log10 Mh = 13.24+0.02-0.02, and blin = 2.08+0.03-0.03. For QSOs, we infer fsat = 3+8-2%, log10 Mh = 12.65+0.09-0.04, and blin = 2.63+0.37-0.26 in redshift range 0.8 < z < 2.1. Using these fits, we generate a large suite of high-fidelity galaxy mocks. We also study the redshift-evolution of the DESI LRG sample from z = 0.4 up to z = 1.1, revealing significant and interesting trends in mean halo mass, linear bias, and satellite fraction.

==> tables/mainMargstat_old.tex <==
\begin{table*}
    \centering
    {\renewcommand{\arraystretch}{1.7}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|c||ccccc|cc|cc|c}
        \hline
        \hline
        \multicolumn{12}{c}{$\mathrm{LRG}\;\;0.4<z<0.6$}\\
        \hline
        Model&Measurements&$\log M_\mathrm{cut}$&$\log M_1$&$\sigma$&$\alpha$&$\kappa$&$\alpha_c$&$\alpha_s$&$f_\mathrm{ic}$&$f_\mathrm{sat}$&$\chi^2/\mathrm{d.o.f}$\\
        \hline
        $\mathrm{Zheng07}+f_\mathrm{ic}$&
        $w_\mathrm{p}+n_z$&
        12.89$^{+0.11}_{-0.09}$&
        14.08$^{+0.10}_{-0.10}$&
        0.27$^{+0.17}_{-0.17}$&
        1.20$^{+0.15}_{-0.19}$&
        0.65$^{+0.45}_{-0.39}$&
        -&-&
        0.92$^{+0.08}_{-0.17}$&
        0.089$_{-0.010}^{+0.013}$&
        4.5/(15-5)\\[3pt]

        % &&(12.95)&(14.11)&(0.36)&(1.26)&(0.48)&(1.00)&&&(0.085)&\\
        \hline

        \makecell[cl]{$\mathrm{Zheng07}+f_\mathrm{ic}$\\$\;\;+\alpha_\mathrm{c}+\alpha_\mathrm{s}$}&
        \xirppi$+n_z$&
        12.79$^{+0.15}_{-0.07}$&
        13.88$^{+0.11}_{-0.11}$&
        0.21$^{+0.11}_{-0.10}$&
        1.07$^{+0.13}_{-0.16}$&
        1.4$^{+0.6}_{-0.5}$&
        0.33$^{+0.05}_{-0.07}$&
        0.80$^{+0.07}_{-0.07}$&
        0.70$^{+0.15}_{-0.09}$&
        0.106$^{+0.011}_{-0.012}$&
        1.10\\

        % &&()&()&()&()&()&()&()&()&()&\\
        \hline
        \multicolumn{12}{c}{$\mathrm{LRG}\;\;0.6<z<0.8$}\\
        \hline

        $\mathrm{Zheng07}+f_\mathrm{ic}$&
        $w_\mathrm{p}+n_z$&
        12.78$_{-0.08}^{+0.10}$&
        13.94$_{-0.11}^{+0.14}$&
        0.23$_{-0.15}^{+0.14}$&
        1.07$_{-0.21}^{+0.16}$&
        0.55$_{-0.34}^{+0.42}$&
        -&-&
        0.89$_{-0.14}^{+0.11}$&
        0.104$_{-0.010}^{+0.013}$&
        19.6/(15-5)\\[3pt]

        % &&(12.76)&(13.91)&(0.22)&(1.18)&(0.36)&(0.85)&&&(0.093)&\\
        \hline

        \makecell[cl]{$\mathrm{Zheng07}+f_\mathrm{ic}$\\$\;\;+\alpha_\mathrm{c}+\alpha_\mathrm{s}$}&
        \xirppi$+n_z$&
        12.64$^{+0.17}_{-0.05}$&
        13.71$^{+0.07}_{-0.07}$&
        0.09$^{+0.09}_{-0.05}$&
        1.18$^{+0.08}_{-0.13}$&
        0.6$^{+0.4}_{-0.2}$&
        0.19$^{+0.06}_{-0.09}$&
        0.95$^{+0.07}_{-0.06}$&
        0.62$^{+0.07}_{-0.06}$&
        0.136$^{+0.011}_{-0.010}$&
        1.05\\

        \hline
        \multicolumn{12}{c}{$\mathrm{QSO}\;\;0.8<z<2.1$}\\
        \hline

        $\mathrm{Zheng07}+f_\mathrm{ic}$&
        $w_\mathrm{p}+n_z$&
        $12.67_{-0.36}^{+0.71}$&
        $15.00_{-0.64}^{+0.62}$&
        $0.58_{-0.35}^{+0.37}$&
        $1.09_{-0.37}^{+0.43}$&
        $0.74_{-0.29}^{+0.41}$&
        -&-&
        $0.041_{-0.016}^{+0.066}$&
        $0.05_{-0.05}^{+0.26}$&
        16.0/(15-5)\\[3pt]

        % &&()&()&()&()&()&()&()&()&()&\\
        \hline
        \makecell[cl]{$\mathrm{Zheng07}+f_\mathrm{ic}$\\$\;\;+\alpha_\mathrm{c}+\alpha_\mathrm{s}$}&
        \xirppi$+n_z$&
        12.2$^{+0.6}_{-0.1}$&
        14.7$^{+0.6}_{-0.6}$&
        0.12$^{+0.28}_{-0.06}$&
        0.8$^{+0.4}_{-0.2}$&
        0.6$^{+0.8}_{-0.2}$&
        1.54$^{+0.17}_{-0.08}$&
        0.6$^{+0.6}_{-0.3}$&
        0.019$^{+0.029}_{-0.004}$&
        0.03$^{+0.08}_{-0.02}$&
        0.96\\

        % &&()&()&()&()&()&()&()&()&()&\\
        \hline
    \end{tabular}%
    }
    }
    \caption{LRG and QSO best-fit parameters, with different models and different measurements. The error bars on the full covariance fits are $1\sigma$ error bars. We also quote the marginalized satellite fraction $f_\mathrm{sat}$ and the sample completeness $f_\mathrm{ic}$.
    }
    \label{tab:LRG_fit1}
\end{table*}

==> tables/oldLrgTable.tex <==
\begin{table*}
\centering
\begin{tabular}{l || cccc | cc}
\hline
\hline
LRG & & & \multicolumn{2}{c}{$0.4 < z < 0.6$} & \multicolumn{2}{c}{$0.6 < z <0.8$}\\
\hline
Parameters & bounds & $\sigma_\mathrm{prior}$ & best-fit (diagonal only) & best-fit (full covariance) & best-fit (diagonal only) & best-fit (full covariance) \\
\hline
$\log M_\mathrm{cut}$ & [12.0, 13.8] & 1.0 & 12.75 & 12.79$^{+0.15}_{-0.07}$ & 12.60 & 12.64$^{+0.17}_{-0.05}$\\
$\log M_1$ & [12.5, 15.5] & 1.0  & 13.92 & 13.88$^{+0.11}_{-0.11}$ & 13.68 & 13.71$^{+0.07}_{-0.07}$ \\
$\sigma$ & [0.0, 3.0] & 0.5 & 0.07 & 0.21$^{+0.11}_{-0.10}$ & 0.10 & 0.09$^{+0.09}_{-0.05}$\\
$\alpha$ & [0.3, 2.0]  & 0.5 & 1.16 & 1.07$^{+0.13}_{-0.16}$ & 1.27 & 1.18$^{+0.08}_{-0.13}$\\
$\kappa$ & [0.0, 3.0] & 1.0 & 1.0 & 1.4$^{+0.6}_{-0.5}$ & 0.26 & 0.6$^{+0.4}_{-0.2}$\\
$\alpha_{c}$ & [0.0, 1.0] & 0.4 & 0.38 & 0.33$^{+0.05}_{-0.07}$& 0.12 & 0.19$^{+0.06}_{-0.09}$\\
$\alpha_{s}$ & [0.5, 2.0] & 0.4 & 0.84 & 0.80$^{+0.07}_{-0.07}$ & 0.93 & 0.95$^{+0.07}_{-0.06}$\\
\hline
$f_\mathrm{sat}$ & - & - & 0.11 & 0.106$^{+0.011}_{-0.012}$& 0.14& 0.136$^{+0.011}_{-0.010}$\\
$f_\mathrm{ic}$ & - & - & 0.69 & 0.70$^{+0.15}_{-0.09}$& 0.56& 0.62$^{+0.07}_{-0.06}$\\
$\log_{10}\overline{M}_h$ & - & - & 13.40 & 13.40$^{+0.02}_{-0.02}$& 13.24& 13.24$^{+0.02}_{-0.02}$\\
\hline
\end{tabular}
\caption{LRG best-fit parameters, with diagonal jackknife errors only and with full covariances. With full covariances, for $z = 0.5$, we get best-fit $\chi^2 = 116$ with 105 degrees of freedom. For $z = 0.8$, we get best-fit $\chi^2 = 111$ with 105 degrees of freedom. The error bars on the full covariance fits are $1\sigma$ error bars. The bottom three rows present the marginalised satellite fraction, the sample completeness, and the average halo mass per galaxy.}
\label{tab:LRG_fit1}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{l || c cc }
\hline
\hline
QSO & & \multicolumn{2}{c}{$0.8<z<2.1$}\\
\hline
Parameters & bounds & best-fit (diagonal only) & best-fit (full covariance) \\
\hline
$\log M_\mathrm{cut}$ & [11.2, 14.0] & 12.74 & 12.2$^{+0.6}_{-0.1}$\\
$\log M_1$ & [12.0, 16.0] & 14.94 & 14.7$^{+0.6}_{-0.6}$ \\
$\sigma$ & [0.0, 3.0] & 0.44 & 0.12$^{+0.28}_{-0.06}$\\
$\alpha$ & [0.3, 2.0] & 0.96 & 0.8$^{+0.4}_{-0.2}$\\
$\kappa$ & [0.0, 3.0] & 0.055 & 0.6$^{+0.8}_{-0.2}$\\
$\alpha_{c}$ & [0.0, 2.0]  & 1.53 & 1.54$^{+0.17}_{-0.08}$\\
$\alpha_{s}$ & [0.0, 2.0]  & 0.16 & 0.6$^{+0.6}_{-0.3}$\\
\hline
$f_\mathrm{sat}$ & -  & 0.02 & 0.03$^{+0.08}_{-0.02}$\\
$f_\mathrm{ic}$ & -  & 0.045 & 0.019$^{+0.029}_{-0.004}$\\
$\log_{10}\overline{M}_h$ & - & 12.75 & 12.65$^{+0.09}_{-0.04}$\\
\hline
\end{tabular}
\caption{QSO best-fit parameters, with diagonal jackknife errors only and with full covariances. The error bars on the full covariance fits are $1\sigma$ error bars. }
\label{tab:QSO_table}
\end{table*}
